Structured Event Reasoning with Large Language Models

Reasoning about real-life events is a unifying challenge in AI and NLP that has profound utility in a variety of domains, while fallacy in high-stake applications could be catastrophic. Able to work with diverse text in these domains, large language models (LLMs) have proven capable of answering questions and solving problems. However, I show that end-to-end LLMs still systematically fail to reason about complex events, and they lack interpretability due to their black-box nature. To address these issues, I propose three general approaches to use LLMs in conjunction with a structured representation of events. The first is a language-based representation involving relations of sub-events that can be learned by LLMs via fine-tuning. The second is a semi-symbolic representation involving states of entities that can be predicted and leveraged by LLMs via few-shot prompting. The third is a fully symbolic representation that can be predicted by LLMs trained with structured data and be executed by symbolic solvers. On a suite of event reasoning tasks spanning common-sense inference and planning, I show that each approach greatly outperforms end-to-end LLMs with more interpretability. These results suggest manners of synergy between LLMs and structured representations for event reasoning and beyond.

==> PackagesLoadedbyTemplate.tex <==
% University of Pennsylvania Ph.D. Dissertation LaTeX Template packages

upennstyle.sty loads the following packages
\begin{itemize}
\item amscd
\item amsfonts
\item amsmath
\item amssymb
\item amsthm
\item appendix
\item array
\item babel
\item blindtext
\item booktabs
\item calc
\item caption
\item csquotes
\item float
\item fontenc
\item geometry 
\item graphicx
\item hyperref
\item multirow
\item parskip
\item pdflscape
\item setspace
\item tabularx
\item titlesec
\item tocloft
\item verbatim
\end{itemize}

sampledissertation.tex loads the following packages
\begin{itemize}
\item upennstyle
\item natbib
\end{itemize}
